Computer-based Deceptive Game Design in Commercial Virtual Reality Games: A Preliminary Investigation

As Virtual Reality (VR) games become more popular, it is crucial to understand how deceptive game design patterns manifest and impact player experiences in this emerging medium. Our study sheds light on the presence and effects of manipulative design techniques in commercial VR games compared to a traditional computer game. We conducted an autoethnography study and developed a VR Deceptive Game Design Assessment Guide based on a critical literature review. Using our guide, we compared how deceptive patterns in a popular computer game are different from two commercial VR titles. While VR's technological constraints, such as battery life and limited temporal manipulation, VR's unique sensory immersion amplified the impact of emotional and sensory deception. Current VR games showed similar but evolved forms of deceptive design compared to the computer game. We forecast more sophisticated player manipulation as VR technology advances. Our findings contribute to a better understanding of how deceptive game design persists and escalates in VR. We highlight the urgent need to develop ethical design guidelines for the rapidly advancing VR games industry.

==> 00-Figure01.tex <==
\begin{figure}[!t]
    \centering
    \begin{minipage}{0.6\textwidth}
       \centering
        % first figure itself
        \includegraphics[width=\textwidth]{DiaryCalendar.pdf}
        %\caption{Overview of VR gameplay sessions and diary entries. Pink indicate days played the game and recorded gameplay sessions videos. While diary entries were regularly written at the end of each gameplay sessions (pink days), blue indicates days that dedicated for writing verbal thoughts, memories, and reflections based on game experience after a certain period of time.}
        %\Description{Overview of VR game play sessions and diary entries. Pink indicate days played the game and recorded gameplay sessions videos. Blue indicates days writing verbal thoughts, memories, and reflections based on game experience after a certain period of time.}
    \end{minipage}\hfill
    \begin{minipage}{0.38\textwidth}
        \centering
        \includegraphics[width=\textwidth]{SampleArtefact.pdf}
        % second figure itself
        %\caption{}
        %\label{fig:diary}
    \end{minipage}
    \caption{Overview of diary study and gameplay recording process and a sample artefact. Pink indicate days played the game and recorded gameplay sessions videos. While diary entries were regularly written at the end of each gameplay sessions (pink days), blue indicates days that dedicated for writing verbal thoughts, memories, and reflections based on game experience after a certain period of time.}
    \Description{{Overview of VR gameplay sessions and diary entries. Pink indicate days played the game and recorded gameplay sessions videos. While diary entries were regularly written at the end of each gameplay sessions (pink days), blue indicates days that dedicated for writing verbal thoughts, memories, and reflections based on game experience after a certain period of time.}
    \label{fig:diary}
\end{figure}

==> 06-Conclusion.tex <==
%\hilda{given the page limit, no need for a standalone conclusion}
